Why Rumors Spread Fast in Social Networks, and How to Stop It

We study a rumor spreading model where individuals are connected via a network structure. Initially, only a small subset of the individuals are spreading a rumor. Each individual who is connected to a spreader, starts spreading the rumor with some probability as a function of their trust in the spreader, quantified by the Jaccard similarity index. Furthermore, the probability that a spreader diffuses the rumor decreases over time until they fully lose their interest and stop spreading. We focus on determining the graph parameters which govern the magnitude and pace that the rumor spreads in this model. We prove that for the rumor to spread to a sizable fraction of the individuals, the network needs to enjoy ``strong'' expansion properties and most nodes should be in ``well-connected'' communities. Both of these characteristics are, arguably, present in real-world social networks up to a certain degree, shedding light on the driving force behind the extremely fast spread of rumors in social networks. Furthermore, we formulate a large range of countermeasures to cease the spread of a rumor. We introduce four fundamental criteria which a countermeasure ideally should possess. We evaluate all the proposed countermeasures by conducting experiments on real-world social networks such as Facebook and Twitter. We conclude that our novel decentralized countermeasures (which are executed by the individuals) generally outperform the previously studied centralized ones (which need to be imposed by a third entity such as the government).

==> tikz.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{crimson2143940}{RGB}{214,39,40}
\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{darkorange25512714}{RGB}{255,127,14}
\definecolor{forestgreen4416044}{RGB}{44,160,44}
\definecolor{gray127}{RGB}{127,127,127}
\definecolor{lightgray204}{RGB}{204,204,204}
\definecolor{mediumpurple148103189}{RGB}{148,103,189}
\definecolor{orchid227119194}{RGB}{227,119,194}
\definecolor{sienna1408675}{RGB}{140,86,75}
\definecolor{steelblue31119180}{RGB}{31,119,180}

\begin{axis}[
% legend pos=outer north east,
legend columns=2,
legend style={
  fill opacity=0.8,
  draw opacity=1,
  text opacity=1,
  at={(0.5,-0.2)},
  anchor=north,
  draw=lightgray204,
},
tick align=outside,
tick pos=left,
x grid style={darkgray176},
xlabel={rounds},
xmin=-3, xmax=63,
xtick style={color=black},
y grid style={darkgray176},
ylabel={fraction of orange nodes},
ymin=-0.0231666254023273, ymax=0.486499133448873,
ytick style={color=black}
]
\addplot [thick, steelblue31119180]
table {%
0 0
1 0
2 0
3 0
4 0
5 0.000247586036147561
6 0.00133696459519683
7 0.00834364941817281
8 0.0226293637038871
9 0.0397375588016836
10 0.0618965090368903
11 0.0848229759841545
12 0.107056202030205
13 0.121564743748453
14 0.132433770735331
15 0.143302797722208
16 0.150928447635553
17 0.156400099034414
18 0.160311958405546
19 0.164124783362218
20 0.167789056697202
21 0.170636296112899
22 0.172319881158703
23 0.173656845753899
24 0.174523396880416
25 0.175142361970785
26 0.175786085664769
27 0.176132706115375
28 0.176231740529834
29 0.176405050755137
30 0.176652636791285
31 0.176875464223818
32 0.176949740034662
33 0.176974498638277
34 0.176999257241892
35 0.176999257241892
36 0.176999257241892
37 0.176999257241892
38 0.176999257241892
39 0.176999257241892
40 0.176999257241892
41 0.176999257241892
42 0.176999257241892
43 0.176999257241892
44 0.176999257241892
45 0.176999257241892
46 0.176999257241892
47 0.176999257241892
48 0.176999257241892
};
\addlegendentry{facebook-$\Delta=1$}
\addplot [thick, darkorange25512714]
table {%
0 0
1 0
2 0
3 0
4 0
5 0.000247586036147561
6 0.00203020549641
7 0.0119584055459272
8 0.029338945283486
9 0.0527605843030453
10 0.066699678138153
11 0.0791284971527606
12 0.0911116613023026
13 0.102971032433771
14 0.11374102500619
15 0.124040604109928
16 0.13295370141124
17 0.140925971775192
18 0.148601138895766
19 0.157910373854915
20 0.165313196335727
21 0.170413468680366
22 0.174028224808121
23 0.176132706115375
24 0.177321119088883
25 0.177791532557564
26 0.178088635800941
27 0.178237187422629
28 0.178336221837088
29 0.178385739044318
30 0.178435256251547
31 0.178509532062392
32 0.178608566476851
33 0.17870760089131
34 0.178757118098539
35 0.178781876702154
36 0.178781876702154
37 0.178781876702154
38 0.178781876702154
39 0.178781876702154
40 0.178781876702154
41 0.178781876702154
42 0.178781876702154
43 0.178781876702154
44 0.178781876702154
45 0.178781876702154
46 0.178781876702154
47 0.178781876702154
48 0.178781876702154
49 0.178781876702154
50 0.178781876702154
51 0.178781876702154
52 0.178781876702154
53 0.178781876702154
54 0.178781876702154
55 0.178781876702154
56 0.178781876702154
57 0.178781876702154
58 0.178781876702154
59 0.178781876702154
60 0.178781876702154
};
\addlegendentry{facebook-$\Delta=2$}
\addplot [thick, forestgreen4416044]
table {%
0 0
1 0
2 0
3 0
4 0
5 0.000247586036147561
6 0.00175786085664769
7 0.00945778658083684
8 0.0272592225798465
9 0.0556078237187423
10 0.0900717999504828
11 0.118544194107452
12 0.149740034662045
13 0.172765536023768
14 0.200371379054221
15 0.227036395147314
16 0.253131963357267
17 0.272839811834613
18 0.28880911116613
19 0.300445654865066
20 0.309234959148304
21 0.316885367665264
22 0.322035157217133
23 0.325377568705125
24 0.327729636048527
25 0.329314186679871
26 0.330131220599158
27 0.330552116860609
28 0.330700668482298
29 0.330799702896757
30 0.330898737311216
31 0.33097301312206
32 0.330997771725675
33 0.330997771725675
34 0.330997771725675
35 0.330997771725675
36 0.330997771725675
37 0.330997771725675
38 0.330997771725675
39 0.330997771725675
40 0.330997771725675
41 0.330997771725675
42 0.330997771725675
43 0.330997771725675
44 0.330997771725675
45 0.330997771725675
46 0.330997771725675
47 0.330997771725675
48 0.330997771725675
49 0.330997771725675
50 0.330997771725675
51 0.330997771725675
52 0.330997771725675
53 0.330997771725675
54 0.330997771725675
};
\addlegendentry{facebook-$\Delta=4$}
\addplot [thick, crimson2143940]
table {%
0 0
1 0
2 0
3 0
4 0
5 0.000247586036147561
6 0.000643723693983659
7 0.00232730873978708
8 0.00849220103986135
9 0.0224808120821986
10 0.0492448625897499
11 0.0880911116613023
12 0.117974746224313
13 0.140777420153503
14 0.161921267640505
15 0.183684080217876
16 0.219683089873731
17 0.263778162911612
18 0.307798960138648
19 0.335008665511265
20 0.359222579846497
21 0.380886358009408
22 0.399801931171082
23 0.413939093835108
24 0.424535776182223
25 0.432730873978708
26 0.438301559792028
27 0.443278039118594
28 0.448502104481307
29 0.453577618222332
30 0.456028719980193
31 0.458182718494677
32 0.460163406783857
33 0.461500371379054
34 0.461995543451349
35 0.462267888091112
36 0.462589749938103
37 0.462763060163407
38 0.462787818767021
39 0.462862094577866
40 0.462961128992325
41 0.463010646199554
42 0.463109680614013
43 0.463233473632087
44 0.463282990839317
45 0.463282990839317
46 0.463332508046546
47 0.463332508046546
48 0.463332508046546
};
\addlegendentry{facebook-$\Delta=8$}
\addplot [thick, mediumpurple148103189]
table {%
0 0
1 0
2 0
3 0
4 0
5 1.22992153100632e-05
6 3.19779598061644e-05
7 0.000134061446879689
8 0.000589132413352028
9 0.00221139891274937
10 0.00670922195163949
11 0.0168093375642634
12 0.0378520650382506
13 0.0703576611812166
14 0.108956288588788
15 0.142001820283866
16 0.166783509212112
17 0.184483309964824
18 0.196536540968686
19 0.204592526996778
20 0.210011561262391
21 0.213923941652523
22 0.216416992595872
23 0.217971613411064
24 0.218930952205249
25 0.219572971244435
26 0.220030502053969
27 0.220281406046294
28 0.220507711607999
29 0.220690969916119
30 0.220821341598406
31 0.220928344771604
32 0.221011979435712
33 0.22108331488451
34 0.22111898260891
35 0.221144810961061
36 0.221159570019433
37 0.221173099156274
38 0.22118047868546
39 0.221194007822301
40 0.221201387351487
41 0.221207536959142
42 0.221212456645266
43 0.221212456645266
44 0.221212456645266
45 0.221212456645266
46 0.221212456645266
47 0.221212456645266
48 0.221212456645266
};
\addlegendentry{twitter-$\Delta=1$}
\addplot [thick, sienna1408675]
table {%
0 0
1 0
2 0
3 0
4 0
5 1.22992153100632e-05
6 4.67370181782402e-05
7 0.000194327601898999
8 0.000817897818119204
9 0.0031904164514304
10 0.00844956091801343
11 0.0200538705630581
12 0.0444776523257816
13 0.081119474577522
14 0.121476889774432
15 0.153111701473446
16 0.174458219565592
17 0.188703170737707
18 0.198439229577153
19 0.204829901852262
20 0.208642658598381
21 0.21126854106708
22 0.212905566624849
23 0.213882124320468
24 0.214423289794111
25 0.214782426881165
26 0.215025951344304
27 0.215180921457211
28 0.215300223845719
29 0.215367869529924
30 0.215418296312695
31 0.215441664821784
32 0.215466263252404
33 0.215479792389246
34 0.215487171918432
35 0.215495781369149
36 0.215503160898335
37 0.21550931050599
38 0.215511770349052
39 0.215514230192114
40 0.215515460113645
41 0.215515460113645
42 0.215515460113645
43 0.215515460113645
44 0.215515460113645
45 0.215515460113645
46 0.215515460113645
47 0.215515460113645
48 0.215515460113645
};
\addlegendentry{twitter-$\Delta=2$}
\addplot [thick, orchid227119194]
table {%
0 0
1 0
2 0
3 0
4 0
5 1.22992153100632e-05
6 5.28866258332718e-05
7 0.000479669397092465
8 0.00180552480751728
9 0.00333308734902713
10 0.00640912109807394
11 0.0144540378323863
12 0.0334304971342828
13 0.0655093105059897
14 0.106224632868423
15 0.148419550832657
16 0.186037930780016
17 0.216993825793914
18 0.240630457776794
19 0.257507441025263
20 0.269039185299978
21 0.276629031067818
22 0.28180208102723
23 0.285395911740831
24 0.287860674488968
25 0.289500159889799
26 0.290476717585418
27 0.291085528743266
28 0.29149386269156
29 0.29171401864561
30 0.291899736796792
31 0.2920190391853
32 0.292101443927877
33 0.292151870710649
34 0.2921776990628
35 0.292198607728827
36 0.292209677022606
37 0.292221976237916
38 0.292235505374757
39 0.292247804590067
40 0.292252724276191
41 0.292255184119253
42 0.292256414040784
43 0.292257643962315
44 0.292257643962315
45 0.292258873883846
46 0.292258873883846
47 0.292258873883846
48 0.292258873883846
49 0.292258873883846
50 0.292258873883846
51 0.292258873883846
52 0.292258873883846
53 0.292258873883846
54 0.292258873883846
};
\addlegendentry{twitter-$\Delta=4$}
\addplot [thick, gray127]
table {%
0 0
1 0
2 0
3 0
4 0
5 1.22992153100632e-05
6 4.55070966472339e-05
7 0.000218926032519125
8 0.00105896243819644
9 0.00423461983125477
10 0.0117691191301995
11 0.0276412564878361
12 0.0579539025410179
13 0.106035224952648
14 0.168569355275133
15 0.236667650603891
16 0.292482719602489
17 0.330110938922097
18 0.354056281209259
19 0.369537303520035
20 0.378951122918358
21 0.38462475094089
22 0.388000885543502
23 0.390156937987356
24 0.391404078419797
25 0.392132191966153
26 0.392558974737412
27 0.392819718101985
28 0.392990677194795
29 0.393091530760337
30 0.393161636287605
31 0.393203453619659
32 0.393239121344058
33 0.393255110323961
34 0.393260030010085
35 0.39326617961774
36 0.393269869382333
37 0.393273559146926
38 0.393273559146926
39 0.393273559146926
40 0.393273559146926
41 0.393273559146926
42 0.393273559146926
};
\addlegendentry{twitter-$\Delta=8$}
\end{axis}

\end{tikzpicture}

==> tikz_community_edges.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}
\tiny
\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{green}{RGB}{0,128,0}
\definecolor{lightgray204}{RGB}{204,204,204}

\begin{axis}[
legend cell align={left},
legend style={
  fill opacity=0.8,
  draw opacity=1,
  text opacity=1,
  at={(0.02,0.97)},
  anchor=north west,
  draw=lightgray204
},
tick align=outside,
tick pos=left,
x grid style={darkgray176},
xlabel={rounds},
xmin=-2.7, xmax=56.7,
xtick style={color=black},
y grid style={darkgray176},
ylabel={fraction of broken edges},
ymin=-1.60494514549972, ymax=33.7038480554941,
ytick style={color=black}
]
\addplot [thick, green]
table {%
0 0
1 0
2 0
3 0.0314434265907403
4 0.0939836593216143
5 0.259197821242882
6 0.5654369893538
7 1.07709829165635
8 1.71859371131468
9 2.39264669472642
10 3.06669967813815
11 3.67204753651894
12 4.2058677890567
13 4.70851695964348
14 4.89977717256747
15 5.01460757613271
16 5.05902451101758
17 5.10344144590245
18 5.16699678138153
19 5.19910869026987
20 5.21824709086408
21 5.25652389205249
22 5.2948006932409
23 5.33307749442931
24 5.43268135677148
25 5.51314681851944
26 5.59361228026739
27 5.65493934142114
28 5.71626640257489
29 5.79779648427829
30 5.8731616736816
31 5.92609556820995
32 5.9790294627383
33 6.03196335726665
34 6.090938351077
35 6.12139143352315
36 6.1518445159693
37 6.18229759841545
38 6.19192869522159
39 6.20155979202773
40 6.21119088883387
41 6.21723198811587
42 6.22327308739787
43 6.22931418667987
44 6.23535528596187
45 6.23535528596187
46 6.23535528596187
47 6.23535528596187
48 6.23535528596187
49 6.23535528596187
50 6.23535528596187
% 51 6.23535528596187
% 52 6.23535528596187
% 53 6.23535528596187
% 54 6.23535528596187
};
\addlegendentry{FB}
\addplot [thick, red]
table {%
0 0
1 0
2 0
3 0
4 0
5 0
6 0.295546454136226
7 1.30308833296436
8 3.24403242073156
9 5.74883526431014
10 8.73185004796694
11 12.0396452906305
12 15.3923880156446
13 18.737642978378
14 21.8726379356997
15 24.7881423265196
16 27.5446756696923
17 29.7925269967776
18 31.06941677121
19 31.7380660713846
20 32.0989029099943
21 32.0989029099943
22 32.0989029099943
23 32.0989029099943
24 32.0989029099943
25 32.0989029099943
26 32.0989029099943
27 32.0989029099943
28 32.0989029099943
29 32.0989029099943
30 32.0989029099943
31 32.0989029099943
32 32.0989029099943
33 32.0989029099943
34 32.0989029099943
35 32.0989029099943
36 32.0989029099943
37 32.0989029099943
38 32.0989029099943
39 32.0989029099943
40 32.0989029099943
41 32.0989029099943
42 32.0989029099943
43 32.0989029099943
44 32.0989029099943
45 32.0989029099943
46 32.0989029099943
47 32.0989029099943
48 32.0989029099943
49 32.0989029099943
50 32.0989029099943
% 51 32.0989029099943
% 52 32.0989029099943
% 53 32.0989029099943
% 54 32.0989029099943
};
\addlegendentry{TW}
\end{axis}

\end{tikzpicture}


==> tikz_community_nodes.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}
\tiny
\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{green}{RGB}{0,128,0}
\definecolor{lightgray204}{RGB}{204,204,204}

\begin{axis}[
legend cell align={left},
legend style={
  fill opacity=0.8,
  draw opacity=1,
  text opacity=1,
  at={(0.02,0.97)},
  anchor=north west,
  draw=lightgray204
},
tick align=outside,
tick pos=left,
x grid style={darkgray176},
xlabel={rounds},
xmin=-2.7, xmax=56.7,
xtick style={color=black},
y grid style={darkgray176},
ylabel={fraction of orange nodes},
ymin=-0.0240963766511697, ymax=0.506023909674563,
ytick style={color=black}
]
\addplot [thick, green]
table {%
0 0
1 0
2 0
3 0
4 0
5 0.000247586036147561
6 0.00200544689279525
7 0.0148056449616242
8 0.0307997028967566
9 0.0506313443921763
10 0.0809358752166378
11 0.121366674919535
12 0.166377816291161
13 0.204877444912107
14 0.223000742758108
15 0.232978460014855
16 0.240356523892052
17 0.247016588264422
18 0.253131963357267
19 0.258702649170587
20 0.262614508541718
21 0.266229264669473
22 0.271478088635801
23 0.277841049764793
24 0.286085664768507
25 0.294280762564991
26 0.298861104233721
27 0.301832136667492
28 0.308318890814558
29 0.316093092349592
30 0.317504332755633
31 0.318692745729141
32 0.31978212428819
33 0.321837088388215
34 0.325278534290666
35 0.327556325823224
36 0.328620945778658
37 0.329834117355781
38 0.330576875464224
39 0.331344392176281
40 0.332631839564249
41 0.334265907402822
42 0.335602871998019
43 0.336840802178757
44 0.339019559296856
45 0.340455558306512
46 0.341198316414954
47 0.34164397128002
48 0.341817281505323
49 0.341941074523397
50 0.341965833127012
% 51 0.342015350334241
% 52 0.342040108937856
% 53 0.342040108937856
% 54 0.342040108937856
};
\addlegendentry{FB}
\addplot [thick, red]
table {%
0 0
1 0
2 0
3 0
4 0
5 1.22992153100632e-05
6 7.01055272673603e-05
7 0.000456300888003345
8 0.00234546035962906
9 0.00945194696578358
10 0.0270705728974491
11 0.0579416033257078
12 0.107873957641502
13 0.176718815339581
14 0.249099697439303
15 0.314685263080215
16 0.368373797751703
17 0.405759722529703
18 0.429852655400586
19 0.444990529604211
20 0.454887708164219
21 0.46153789388237
22 0.465867217671513
23 0.468794430915308
24 0.470884067596487
25 0.472351363982978
26 0.4736255626891
27 0.474885002336851
28 0.476006690773129
29 0.47707180281898
30 0.477920448675374
31 0.478748185865742
32 0.47957715297764
33 0.48026098934888
34 0.480704991021573
35 0.480948515484712
36 0.481103485597619
37 0.481200649398568
38 0.481318721865545
39 0.481413425823432
40 0.481536417976533
41 0.481653260521979
42 0.481722136127715
43 0.481761493616707
44 0.481819299928665
45 0.481867266868374
46 0.481880796005215
47 0.481889405455932
48 0.481896784985118
49 0.481906624357366
50 0.481917693651145
% 51 0.4819238432588
% 52 0.481927533023393
% 53 0.481927533023393
% 54 0.481927533023393
};
\addlegendentry{TW}
\end{axis}

\end{tikzpicture}


==> tikz_green_node.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}
\tiny
\definecolor{crimson2143940}{RGB}{214,39,40}
\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{darkorange25512714}{RGB}{255,127,14}
\definecolor{forestgreen4416044}{RGB}{44,160,44}
\definecolor{gray127}{RGB}{127,127,127}
\definecolor{lightgray204}{RGB}{204,204,204}
\definecolor{mediumpurple148103189}{RGB}{148,103,189}
\definecolor{orchid227119194}{RGB}{227,119,194}
\definecolor{sienna1408675}{RGB}{140,86,75}
\definecolor{steelblue31119180}{RGB}{31,119,180}

\begin{axis}[
legend cell align={left},
legend style={
  fill opacity=0.8,
  draw opacity=1,
  text opacity=1,
  at={(0.01,0.99)},
  anchor=north west,
  draw=lightgray204
},
tick align=outside,
tick pos=left,
x grid style={darkgray176},
xlabel={rounds},
xmin=-2.7, xmax=52.5,
xtick style={color=black},
y grid style={darkgray176},
ylabel={fraction of orange nodes},
ytick style={color=black}
]
\addplot [thick, steelblue31119180, dashed]
table {%
0 0
1 0
2 0
3 0
4 0
5 0.000247586036147561
6 0.00133696459519683
7 0.00834364941817281
8 0.0226293637038871
9 0.0397375588016836
10 0.0618965090368903
11 0.0848229759841545
12 0.107056202030205
13 0.121564743748453
14 0.132433770735331
15 0.143302797722208
16 0.150928447635553
17 0.156400099034414
18 0.160311958405546
19 0.164124783362218
20 0.167789056697202
21 0.170636296112899
22 0.172319881158703
23 0.173656845753899
24 0.174523396880416
25 0.175142361970785
26 0.175786085664769
27 0.176132706115375
28 0.176231740529834
29 0.176405050755137
30 0.176652636791285
31 0.176875464223818
32 0.176949740034662
33 0.176974498638277
34 0.176999257241892
35 0.176999257241892
36 0.176999257241892
37 0.176999257241892
38 0.176999257241892
39 0.176999257241892
40 0.176999257241892
41 0.176999257241892
42 0.176999257241892
43 0.176999257241892
44 0.176999257241892
45 0.176999257241892
46 0.176999257241892
47 0.176999257241892
48 0.176999257241892
%*************************
49 0.176999257241892
50 0.176999257241892
% 51 0.176999257241892
% 52 0.176999257241892
% 53 0.176999257241892
% 54 0.176999257241892
% 55 0.176999257241892
% 56 0.176999257241892
% 57 0.176999257241892
% 58 0.176999257241892
% 59 0.176999257241892
% 60 0.176999257241892
};
\addlegendentry{FB-$\tau=1$}
\addplot [thick, darkorange25512714]
table {%
0 0
1 0
2 0
3 0
4 0
5 0.000247586036147561
6 0.00203020549641
7 0.0119584055459272
8 0.029338945283486
9 0.0527605843030453
10 0.066699678138153
11 0.0791284971527606
12 0.0911116613023026
13 0.102971032433771
14 0.11374102500619
15 0.124040604109928
16 0.13295370141124
17 0.140925971775192
18 0.148601138895766
19 0.157910373854915
20 0.165313196335727
21 0.170413468680366
22 0.174028224808121
23 0.176132706115375
24 0.177321119088883
25 0.177791532557564
26 0.178088635800941
27 0.178237187422629
28 0.178336221837088
29 0.178385739044318
30 0.178435256251547
31 0.178509532062392
32 0.178608566476851
33 0.17870760089131
34 0.178757118098539
35 0.178781876702154
36 0.178781876702154
37 0.178781876702154
38 0.178781876702154
39 0.178781876702154
40 0.178781876702154
41 0.178781876702154
42 0.178781876702154
43 0.178781876702154
44 0.178781876702154
45 0.178781876702154
46 0.178781876702154
47 0.178781876702154
48 0.178781876702154
49 0.178781876702154
50 0.178781876702154
% 51 0.178781876702154
% 52 0.178781876702154
% 53 0.178781876702154
% 54 0.178781876702154
% 55 0.178781876702154
% 56 0.178781876702154
% 57 0.178781876702154
% 58 0.178781876702154
% 59 0.178781876702154
% 60 0.178781876702154
};
\addlegendentry{FB-$\tau=2$}
\addplot [thick, forestgreen4416044]
table {%
0 0
1 0
2 0
3 0
4 0
5 0.000247586036147561
6 0.00175786085664769
7 0.00945778658083684
8 0.0272592225798465
9 0.0556078237187423
10 0.0900717999504828
11 0.118544194107452
12 0.149740034662045
13 0.172765536023768
14 0.200371379054221
15 0.227036395147314
16 0.253131963357267
17 0.272839811834613
18 0.28880911116613
19 0.300445654865066
20 0.309234959148304
21 0.316885367665264
22 0.322035157217133
23 0.325377568705125
24 0.327729636048527
25 0.329314186679871
26 0.330131220599158
27 0.330552116860609
28 0.330700668482298
29 0.330799702896757
30 0.330898737311216
31 0.33097301312206
32 0.330997771725675
33 0.330997771725675
34 0.330997771725675
35 0.330997771725675
36 0.330997771725675
37 0.330997771725675
38 0.330997771725675
39 0.330997771725675
40 0.330997771725675
41 0.330997771725675
42 0.330997771725675
43 0.330997771725675
44 0.330997771725675
45 0.330997771725675
46 0.330997771725675
47 0.330997771725675
48 0.330997771725675
49 0.330997771725675
50 0.330997771725675
% 51 0.330997771725675
% 52 0.330997771725675
% 53 0.330997771725675
% 54 0.330997771725675
%********************
% 55 0.330997771725675
% 56 0.330997771725675
% 57 0.330997771725675
% 58 0.330997771725675
% 59 0.330997771725675
% 60 0.330997771725675
};
\addlegendentry{FB-$\tau=4$}
\addplot [thick, crimson2143940]
table {%
0 0
1 0
2 0
3 0
4 0
5 0.000247586036147561
6 0.000643723693983659
7 0.00232730873978708
8 0.00849220103986135
9 0.0224808120821986
10 0.0492448625897499
11 0.0880911116613023
12 0.117974746224313
13 0.140777420153503
14 0.161921267640505
15 0.183684080217876
16 0.219683089873731
17 0.263778162911612
18 0.307798960138648
19 0.335008665511265
20 0.359222579846497
21 0.380886358009408
22 0.399801931171082
23 0.413939093835108
24 0.424535776182223
25 0.432730873978708
26 0.438301559792028
27 0.443278039118594
28 0.448502104481307
29 0.453577618222332
30 0.456028719980193
31 0.458182718494677
32 0.460163406783857
33 0.461500371379054
34 0.461995543451349
35 0.462267888091112
36 0.462589749938103
37 0.462763060163407
38 0.462787818767021
39 0.462862094577866
40 0.462961128992325
41 0.463010646199554
42 0.463109680614013
43 0.463233473632087
44 0.463282990839317
45 0.463282990839317
46 0.463332508046546
47 0.463332508046546
48 0.463332508046546
%******************
49 0.463332508046546
50 0.463332508046546
% 51 0.463332508046546
% 52 0.463332508046546
% 53 0.463332508046546
% 54 0.463332508046546
% 55 0.463332508046546
% 56 0.463332508046546
% 57 0.463332508046546
% 58 0.463332508046546
% 59 0.463332508046546
% 60 0.463332508046546
};
\addlegendentry{FB-$\tau=8$}
\addplot [thick, mediumpurple148103189, dashed]
table {%
0 0
1 0
2 0
3 0
4 0
5 1.22992153100632e-05
6 3.19779598061644e-05
7 0.000134061446879689
8 0.000589132413352028
9 0.00221139891274937
10 0.00670922195163949
11 0.0168093375642634
12 0.0378520650382506
13 0.0703576611812166
14 0.108956288588788
15 0.142001820283866
16 0.166783509212112
17 0.184483309964824
18 0.196536540968686
19 0.204592526996778
20 0.210011561262391
21 0.213923941652523
22 0.216416992595872
23 0.217971613411064
24 0.218930952205249
25 0.219572971244435
26 0.220030502053969
27 0.220281406046294
28 0.220507711607999
29 0.220690969916119
30 0.220821341598406
31 0.220928344771604
32 0.221011979435712
33 0.22108331488451
34 0.22111898260891
35 0.221144810961061
36 0.221159570019433
37 0.221173099156274
38 0.22118047868546
39 0.221194007822301
40 0.221201387351487
41 0.221207536959142
42 0.221212456645266
43 0.221212456645266
44 0.221212456645266
45 0.221212456645266
46 0.221212456645266
47 0.221212456645266
48 0.221212456645266
%********************
49 0.221212456645266
50 0.221212456645266
% 51 0.221212456645266
% 52 0.221212456645266
% 53 0.221212456645266
% 54 0.221212456645266
% 55 0.221212456645266
% 56 0.221212456645266
% 57 0.221212456645266
% 58 0.221212456645266
% 59 0.221212456645266
% 60 0.221212456645266
};
\addlegendentry{TW-$\tau=1$}
\addplot [thick, sienna1408675]
table {%
0 0
1 0
2 0
3 0
4 0
5 1.22992153100632e-05
6 4.67370181782402e-05
7 0.000194327601898999
8 0.000817897818119204
9 0.0031904164514304
10 0.00844956091801343
11 0.0200538705630581
12 0.0444776523257816
13 0.081119474577522
14 0.121476889774432
15 0.153111701473446
16 0.174458219565592
17 0.188703170737707
18 0.198439229577153
19 0.204829901852262
20 0.208642658598381
21 0.21126854106708
22 0.212905566624849
23 0.213882124320468
24 0.214423289794111
25 0.214782426881165
26 0.215025951344304
27 0.215180921457211
28 0.215300223845719
29 0.215367869529924
30 0.215418296312695
31 0.215441664821784
32 0.215466263252404
33 0.215479792389246
34 0.215487171918432
35 0.215495781369149
36 0.215503160898335
37 0.21550931050599
38 0.215511770349052
39 0.215514230192114
40 0.215515460113645
41 0.215515460113645
42 0.215515460113645
43 0.215515460113645
44 0.215515460113645
45 0.215515460113645
46 0.215515460113645
47 0.215515460113645
48 0.215515460113645
%*******************
49 0.215515460113645
50 0.215515460113645
% 51 0.215515460113645
% 52 0.215515460113645
% 53 0.215515460113645
% 54 0.215515460113645
% 55 0.215515460113645
% 56 0.215515460113645
% 57 0.215515460113645
% 58 0.215515460113645
% 59 0.215515460113645
% 60 0.215515460113645
};
\addlegendentry{TW-$\tau=2$}
\addplot [thick, orchid227119194]
table {%
0 0
1 0
2 0
3 0
4 0
5 1.22992153100632e-05
6 5.28866258332718e-05
7 0.000479669397092465
8 0.00180552480751728
9 0.00333308734902713
10 0.00640912109807394
11 0.0144540378323863
12 0.0334304971342828
13 0.0655093105059897
14 0.106224632868423
15 0.148419550832657
16 0.186037930780016
17 0.216993825793914
18 0.240630457776794
19 0.257507441025263
20 0.269039185299978
21 0.276629031067818
22 0.28180208102723
23 0.285395911740831
24 0.287860674488968
25 0.289500159889799
26 0.290476717585418
27 0.291085528743266
28 0.29149386269156
29 0.29171401864561
30 0.291899736796792
31 0.2920190391853
32 0.292101443927877
33 0.292151870710649
34 0.2921776990628
35 0.292198607728827
36 0.292209677022606
37 0.292221976237916
38 0.292235505374757
39 0.292247804590067
40 0.292252724276191
41 0.292255184119253
42 0.292256414040784
43 0.292257643962315
44 0.292257643962315
45 0.292258873883846
46 0.292258873883846
47 0.292258873883846
48 0.292258873883846
49 0.292258873883846
50 0.292258873883846
% 51 0.292258873883846
% 52 0.292258873883846
% 53 0.292258873883846
% 54 0.292258873883846
%*******************
% 55 0.292258873883846
% 56 0.292258873883846
% 57 0.292258873883846
% 58 0.292258873883846
% 59 0.292258873883846
% 60 0.292258873883846
};
\addlegendentry{TW-$\tau=4$}
\addplot [thick, gray127]
table {%
0 0
1 0
2 0
3 0
4 0
5 1.22992153100632e-05
6 4.55070966472339e-05
7 0.000218926032519125
8 0.00105896243819644
9 0.00423461983125477
10 0.0117691191301995
11 0.0276412564878361
12 0.0579539025410179
13 0.106035224952648
14 0.168569355275133
15 0.236667650603891
16 0.292482719602489
17 0.330110938922097
18 0.354056281209259
19 0.369537303520035
20 0.378951122918358
21 0.38462475094089
22 0.388000885543502
23 0.390156937987356
24 0.391404078419797
25 0.392132191966153
26 0.392558974737412
27 0.392819718101985
28 0.392990677194795
29 0.393091530760337
30 0.393161636287605
31 0.393203453619659
32 0.393239121344058
33 0.393255110323961
34 0.393260030010085
35 0.39326617961774
36 0.393269869382333
37 0.393273559146926
38 0.393273559146926
39 0.393273559146926
40 0.393273559146926
41 0.393273559146926
42 0.393273559146926
%********************
43 0.393273559146926
44 0.393273559146926
45 0.393273559146926
46 0.393273559146926
47 0.393273559146926
48 0.393273559146926
49 0.393273559146926
50 0.393273559146926
% 51 0.393273559146926
% 52 0.393273559146926
% 53 0.393273559146926
% 54 0.393273559146926
% 55 0.393273559146926
% 56 0.393273559146926
% 57 0.393273559146926
% 58 0.393273559146926
% 59 0.393273559146926
% 60 0.393273559146926
};
\addlegendentry{TW-$\tau=8$}
\end{axis}

\end{tikzpicture}
